MRAMG-Bench: A Comprehensive Benchmark for Advancing Multimodal Retrieval-Augmented Multimodal Generation

Recent advances in Retrieval-Augmented Generation (RAG) have significantly improved response accuracy and relevance by incorporating external knowledge into Large Language Models (LLMs). However, existing RAG methods primarily focus on generating text-only answers, even in Multimodal Retrieval-Augmented Generation (MRAG) scenarios, where multimodal elements are retrieved to assist in generating text answers. To address this, we introduce the Multimodal Retrieval-Augmented Multimodal Generation (MRAMG) task, in which we aim to generate multimodal answers that combine both text and images, fully leveraging the multimodal data within a corpus. Despite growing attention to this challenging task, a notable lack of a comprehensive benchmark persists for effectively evaluating its performance. To bridge this gap, we provide MRAMG-Bench, a meticulously curated, human-annotated benchmark comprising 4,346 documents, 14,190 images, and 4,800 QA pairs, distributed across six distinct datasets and spanning three domains: Web, Academia, and Lifestyle. The datasets incorporate diverse difficulty levels and complex multi-image scenarios, providing a robust foundation for evaluating the MRAMG task. To facilitate rigorous evaluation, MRAMG-Bench incorporates a comprehensive suite of both statistical and LLM-based metrics, enabling a thorough analysis of the performance of generative models in the MRAMG task. Additionally, we propose an efficient and flexible multimodal answer generation framework that can leverage LLMs/MLLMs to generate multimodal responses. Our datasets and complete evaluation results for 11 popular generative models are available at https://github.com/MRAMG-Bench/MRAMG.

==> SIG_Statistics.tex <==
\section{Data Statistics}
\label{sec:statistics}

The MRAMG-Bench, summarized in Table~\ref{tab:statistics}, comprises 4,800 QA pairs across three distinct domains: Web Data, Academic Data, and Lifestyle Data. 
It integrates six datasets—\textbf{MRAMG-Wit}, \textbf{MRAMG-Wiki}, \textbf{MRAMG-Web}, \textbf{MRAMG-Arxiv}, \textbf{MRAMG-Recipe}, and \textbf{MRAMG-Manual}—containing 4,346 documents and 14,190 images, with tasks categorized into three difficulty levels. 
Datasets like MRAMG-Recipe and MRAMG-Manual feature longer texts and higher image density, posing greater challenges compared to others.
The benchmark's query distribution captures varying levels of complexity:
Single-image QA primarily involves direct image-text associations.
Two-image QA requires comparative analysis or step-wise reasoning.
Three+ image QA focuses on complex multi-step processes.
Text-only QA emphasizes pure textual reasoning and serves to evaluate the model's ability to exclude irrelevant images when they are not required.

\begin{table*}[htbp]
  \centering
  \caption{The statistics of MRAMG-Bench. Multimodal Element Density refers to the proportion of images to text within a document, indicating image density relative to document length.}
  \vspace{-1mm}
    \resizebox{0.9\textwidth}{!}{
    \begin{tabular}{lccccccc}
    \toprule
    \textbf{DATASETS} & \textbf{MRAMG-Wit} & \textbf{MRAMG-Wiki} & \textbf{MRAMG-Web} & \textbf{MRAMG-Arxiv} & \textbf{MRAMG-Recipe} & \textbf{MRAMG-Manual} & \textbf{Overall} \\
    \midrule
    \textbf{Difficulty Level} & 1     & 1     & 1     & 2     & 3     & 3     & 2.15 \\
    \textbf{Queries} & 600   & 500   & 750   & 200   & 2360  & 390   & 4800 \\
    \textbf{Documents} & 639   & 538   & 1500  & 101   & 1528  & 40    & 4346 \\
    \textbf{Images} & 639   & 538   & 1500  & 337   & 8569  & 2607  & 14190 \\
    \textbf{Avg Images Per Doc} & 1.00  & 1.00  & 1.00  & 3.34  & 5.61  & 65.18 & 3.27 \\
    \textbf{Avg Length Per Doc} & 532.31 & 865.28 & 98.42 & 853.5 & 485.22 & 6365.4 & 468.37 \\
    \textbf{Multimodal Element Density} & 1.88$\times 10^{-3}$ & 1.16$\times 10^{-3}$ & 1.02$\times 10^{-2}$ & 3.91$\times 10^{-3}$ & 1.16$\times 10^{-2}$ & 1.02$\times 10^{-2}$ & 6.98$\times 10^{-3}$ \\
    \textbf{Text-Only QA} & 0     & 0     & 0     & 0     & 92    & 40    & 132 \\
    \textbf{Single-Image QA} & 600   & 500   & 0     & 184   & 1481  & 92    & 2858 \\
    \textbf{Two-Image QA} & 0     & 0     & 750   & 12    & 60    & 126   & 948 \\
    \textbf{Three+ Images QA} & 0     & 0     & 0     & 3     & 727   & 132   & 862 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:statistics}%
\end{table*}%



